TAPS: Connecting Certified and Adversarial Training

Training certifiably robust neural networks remains a notoriously hard problem. On one side, adversarial training optimizes under-approximations of the worst-case loss, which leads to insufficient regularization for certification, while on the other, sound certified training methods optimize loose over-approximations, leading to over-regularization and poor (standard) accuracy. In this work we propose TAPS, an (unsound) certified training method that combines IBP and PGD training to yield precise, although not necessarily sound, worst-case loss approximations, reducing over-regularization and increasing certified and standard accuracies. Empirically, TAPS achieves a new state-of-the-art in many settings, e.g., reaching a certified accuracy of $22\%$ on TinyImageNet for $\ell_\infty$-perturbations with radius $\epsilon=1/255$. We make our implementation and networks public at https://github.com/eth-sri/taps.

==> Makefile <==
# Makefile, allowing to
# - compile
# - test
# - clean
# - run in docker
# For details, see targets defined below
#
# USAGE, for example: make pdf

#####################
# REQUIRED PACKAGES #
#####################

# For instructions on how to set up your system to run all commands here, follow
# https://hub.docker.com/repository/docker/ethsrilab/latex-plus

##############
# PARAMETERS #
##############

# main
OUTPUTDIR := lqa-output
NAME := main
SUBMISSION := submission
SUPPLEMENT := submission_supplement

# special
OVERFULL := $(NAME)_overfull
GRAY := $(NAME)_gray

# submission
SUBMISSIONDIR := final_submission
ZIP := submission.zip

# log
LATEXMKDIR := $(OUTPUTDIR)/latexmk
LOG := $(LATEXMKDIR)/$(NAME).log
SHORTLOG := $(OUTPUTDIR)/$(NAME)-short.log
OVERFULLOUTPUTDIR := $(OUTPUTDIR)/overfull

LOGFILES := *.aux *.bbl *.log *.bcf  *.blg *.lot *.toc *.swp *.gz *.out *.ttt *.fls *.fdb_latexmk

# scripts

SCRIPTDIR := lqa/scripts

#############
# COMPILING #
#############

LATEX         := ./lqa/latex.sh $(NAME).tex $(LATEXMKDIR)
LATEXOVERFULL := ./lqa/latex.sh $(OVERFULL).tex $(OVERFULLOUTPUTDIR)

##########
# OTHERS #
##########

# latex code to enable marking overfull areas
OVERFULLFILECONTENT := \def\isoverfull{1} \input{$(NAME).tex}

########
# PDFS #
########

.DEFAULT_GOAL := pdf

.PHONY: pdf
pdf:
	@echo "\n> COMPILING pdf..."
	$(LATEX)
	@cp $(LATEXMKDIR)/$(NAME).pdf $(OUTPUTDIR)
	@cp $(LATEXMKDIR)/$(NAME).pdf .
	@cp $(LOG) $(OUTPUTDIR)

.PHONY: overfull
overfull:
	@echo "\n> COMPILING OVERFULL pdf..."
	echo "$(OVERFULLFILECONTENT)" > $(OVERFULL).tex
	$(LATEXOVERFULL)
	@cp $(OVERFULLOUTPUTDIR)/$(OVERFULL).pdf $(OUTPUTDIR)
	rm $(OVERFULL).tex # cleanup

# make split: builds the whole paper and splits it into submission and supplementary material
.PHONY: split
split: pdf
	python $(SCRIPTDIR)/pages.py --action split

.PHONY: gray
gray: pdf
	@echo "\n> Producing GRAYSCALE version to $(OUTPUTDIR)/$(GRAY).pdf..."
	gs -sOutputFile=$(OUTPUTDIR)/$(GRAY).pdf -sDEVICE=pdfwrite -sColorConversionStrategy=Gray -dProcessColorModel=/DeviceGray -dCompatibilityLevel=1.4 -qQUIET -dNOPAUSE -dBATCH $(OUTPUTDIR)/$(NAME).pdf

# produce better log files
.PHONY: log
log: pdf
	pplatex -i $(LOG) > $(SHORTLOG)

.PHONY: printlog
printlog: log
	cat $(SHORTLOG)


###############
# CONVENIENCE #
###############

.PHONY: check
check: pdf log
	python $(SCRIPTDIR)/checks.py

.PHONY: all
all: pdf split gray check log overfull

#########
# CLEAN #
#########

.PHONY: clean
clean:
	@echo "\n> CLEANING temporary files..."
	cd $(OUTPUTDIR) && rm -f $(LOGFILES) || true
	rm -f $(LOGFILES) || true
	rm -r -f $(LATEXMKDIR) $(OVERFULLOUTPUTDIR) || true
	rm -r -f $(OUTPUTDIR)/script-logs/*.log* || true

# make cleanall: remove all produced files
.PHONY: cleanall
cleanall: clean
	@echo "\n> CLEANING PDFs..."
	rm -f *.pdf || true
	rm -f $(OUTPUTDIR)/*.pdf || true
	rm -r -f $(SUBMISSIONDIR) || true

##############
# SUBMISSION #
##############

.PHONY: abstract
abstract:
	python $(SCRIPTDIR)/abstract.py

# prepare a submission: produce PDFs and ZIP
.PHONY: submission
submission: split check
	@echo "\n> PREPARING submission in directory $(OUTPUTDIR)..."
	rm -r -f $(SUBMISSIONDIR)
	mkdir $(SUBMISSIONDIR)
	cp $(OUTPUTDIR)/$(SUBMISSION).pdf $(SUBMISSIONDIR)
	cp $(OUTPUTDIR)/$(SUPPLEMENT).pdf $(SUBMISSIONDIR)
	cp $(LATEXMKDIR)/$(NAME).bbl $(SUBMISSIONDIR)

# zip the whole directory and place the result in /submission
.PHONY: zip
zip: submission
	@echo "\n> ZIPPING directory..."
	@rm -f $(SUBMISSIONDIR)/$(ZIP)
	zip --quiet -r $(SUBMISSIONDIR)/$(ZIP) . -x /.git* /$(OUTPUTDIR)* /$(SUBMISSIONDIR)/*.zip

##########
# DOCKER #
##########

DOCKER := ./lqa/docker.sh


PAPERDIR := $$(pwd)
IMAGE := ethsrilab/latex-plus:version-4.0
CONTAINER := latex-plus-container
RUN := $(DOCKER) run \
		-it \
		--name $(CONTAINER) \
		--workdir="/paper" \
		-v $(PAPERDIR):/paper \
		$(IMAGE)

# launch a docker container using the image, which will provide a shell in the container
.PHONY: docker-run
docker-run: clean-container
	$(RUN)

# check for updates and remove the created docker container
.PHONY: clean-container
clean-container:
	$(DOCKER) pull $(IMAGE)
	$(DOCKER) rm /$(CONTAINER) 2>/dev/null || true

# all above commands, run in docker
.PHONY: docker-all
docker-all: clean-container
	$(RUN) make all

.PHONY: docker-pdf
docker-pdf: clean-container
	$(RUN) make pdf

.PHONY: docker-overfull
docker-overfull: clean-container
	$(RUN) make overfull

.PHONY: docker-split
docker-split: clean-container
	$(RUN) make split

.PHONY: docker-gray
docker-gray: clean-container
	$(RUN) make gray

.PHONY: docker-check
docker-check: clean-container
	$(RUN) make check

.PHONY: docker-zip
docker-zip: clean-container
	$(RUN) make zip
	
.PHONY: docker-abstract
docker-abstract: clean-container
	$(RUN) make abstract



==> figures/lqa/inkscape-header.tex <==
% Description: Convenience header for usage with inkscape
%
% Usage:
% - Open inkscape
% - Extensions -> TexText
% - Select this header as "Preamble File"
%
% Configure:
% - Comment out the appropriate packages (depending on your template)

%%%%%%%
% ACM %
%%%%%%%
% Conferences with this template
% - PLDI: Conference on Programming Language Design and Implementation
% - POPL: Principles of Programming Languages
% - CCS: Conference on Computer and Communications Security

% \usepackage[tt=false, type1=true]{libertine}
% \usepackage[libertine]{newtxmath}
% \usepackage[T1]{fontenc}

%%%%%%%%%%%%%%%%%%%%%
% ACM with beramono %
%%%%%%%%%%%%%%%%%%%%%
% has a nice monospace font

\usepackage[tt=false, type1=true]{libertine}
\usepackage[libertine]{newtxmath}
\usepackage[scaled=0.8]{beramono} % necessary for nice font in code
\usepackage[T1]{fontenc}

%%%%%%%%%%%%%%%%%
% IEEE standard %
%%%%%%%%%%%%%%%%%
% Conferences with this template:
% - S&P: Symposium on Security and Privacy

% \usepackage{mathptmx}
% \usepackage[T1]{fontenc}

%%%%%%%%%%%%%%%%%%%%%%
% IEEE no times math %
%%%%%%%%%%%%%%%%%%%%%%
% has nicer math

% \usepackage{times}
% \usepackage[T1]{fontenc}


==> headers/lqa/abbreviations.tex <==
% Description: This file defines commands for common abbreviations
%
% Usage: \input{headers/lqa/abbreviations}

% The Backslash between `.` and ` ` is needed to ensure the white-space is an
% inter-word space, not a inter-sentence space.
%
% Details:
% - https://tex.stackexchange.com/questions/2229/is-a-period-after-an-abbreviation-the-same-as-an-end-of-sentence-period
% - https://stackoverflow.com/questions/2024338/latex-sometimes-puts-too-much-or-too-little-space-after-periods/2024341

\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }
\newcommand{\etc}{etc.}
\newcommand{\cp}{{cp.\ }}
\newcommand{\nth}[1]{$#1^\text{th}$}
\newcommand{\wrt}{{w.r.t.\ }}

==> headers/lqa/acronyms.tex <==
% Description: This file defines acronyms.
%
% Usage: Adapt the list of acronyms below

%%%%%%%%%
% SETUP %
%%%%%%%%%
% import relevant package

\usepackage{acro} % for \ac

%%%%%%%%%%%%%%%%%%%%%%
%  PROJECT-SPECIFIC  %
%%%%%%%%%%%%%%%%%%%%%%
% adapt the following list of acronyms as required

\DeclareAcronym{cli} {
    short = CLI,
    long = Command Line Interface,
    class = abbrev
}

==> lqa/scripts/tests/abstract/header.tex <==
%%%%%%%%%%%%%%%%%
% ABBREVIATIONS %
%%%%%%%%%%%%%%%%%


\newcommand{\eg}{e.g., }
\newcommand{\tool}[0]{\emph{Sometool}\xspace}


==> lqa/scripts/tests/header/cmd.tex <==
abc

\newcommand{\cmd}[0]{cmd}


==> lqa/scripts/tests/header/package.tex <==
abc

\usepackage{abc}


==> lqa/scripts/tests/helpers/main.tex <==
x1
% x2
x3 % x4
x5 \% x6
x7\begin{comment}
x8
\end{comment}x9
x10


==> lqa/scripts/tests/hyphenation/check.tex <==
These occurrences should be fine:

We compute it in constant-time successfully.
We achieve state-of-the-art results.
May hyphenated words may occur at sentence-end?
Hyphenated words may occur at sentence-end.
Hyphenated words may occur at sentence-end!
single-occurrence
occurrence-one occurrence-two
multiple real-worlds

These occurrences should be reported:

We should not write constant time here.
single occurrence
We should not write state-of-the art.


==> lqa/scripts/tests/hyphenation/parse.tex <==
We compute it in constant-time successfully.

We achieve state-of-the-art results.

May hyphenated words may occur at sentence-end?

Hyphenated words may occur at sentence-end.

Hyphenated words may occur at sentence-end!

single-occurrence

occurrence-one occurrence-two

multiple real-worlds

should ignore this: $a-b$

==> lqa/scripts/tests/merge_msgs/merge_msgs.tex <==
Hello world

<<<<<<< HEAD
this is some content to mess with
content to append

=======
totally different content to merge later
>>>>>>> 0489das287d4639d049dddas
that's it


==> lqa/scripts/tests/parse_latex/parser-body.tex <==
\section{My section}

Hello world! This is just an example text that spans multiple lines,
which we can hopefully parse correctly. Even the \emph{third} line should
work if the developers did a good job.

Also a second paragraph goes here. We present \systemname, the first tool
to automatically perform great tasks.

\paragraph{First step} Read this fancy paragraph that even contains
math $x < 3$ in it! There is some continuation of this text, which
should be merged together with part of the text that comes before
the inlined math.

The following formula
\[
    e = mc^2    
\]
is inlined into a sentence.

\begin{figure}
    \centering
    This is a figure content
    \caption{This is a caption}\label{fig:sample-label}
\end{figure}

\begin{enumerate}
    \item First item containing \emph{emphasis} in it % and a comment
          and continues here
    \item Second item
\end{enumerate}

==> lqa/scripts/tests/parse_latex/parser-header.tex <==
\usepackage{xcolor} % for definecolor
\usepackage{amsthm, amsmath}

\newcommand{\systemname}[0]{MySystem}
\newcommand{\eg}[1]{\emph{e.g.,~}}


==> lqa/scripts/tests/references/eqref.tex <==
abc \eqref{def}


==> lqa/scripts/tests/references/ref.tex <==
abc \ref{def}


==> lqa/scripts/tests/unreferenced_floats/floats.tex <==
\section{My section}\label{sec:section}
Hello! We are now referencing \cref{fig:example} and also \cref{tab:example}, but nothing else.

\lstinputlisting[caption={Example code.},label=lst:example]{inexistent.java}

\begin{figure}
    Test
    \caption{Some caption}\label{fig:example}
\end{figure}

\begin{table}
    Test
    \caption{Some caption}
    \label{tab:example}
\end{table}

\begin{figure}
    Test
    \caption{Some caption}
    \label{fig:example_missing}
\end{figure}

\begin{table}
    Test
    \caption{Some caption}\label{tab:example_missing}
\end{table}

==> tables/results_sort_net.tex <==
\begin{wraptable}[8]{r}{0.48 \textwidth}
	\centering
	\vspace{-3mm}
    \caption{Comparison of natural and certified accuracy [\%] to \sortnet \citep{ZhangJHW22}.}
	\vspace{-1mm}
	\resizebox{0.95\linewidth}{!}{
		\renewcommand{\arraystretch}{1.0}
		\begin{threeparttable}
			\begin{tabular}{@{}lccccc@{}}
				\toprule
				\multirow{2.5}{*}{Dataset} & \multirow{2.5}{*}{$\epsilon$} & \multicolumn{2}{c}{\sortnet} & \multicolumn{2}{c}{\toolp (\textbf{ours})} \\
				\cmidrule(rl){3-4}				\cmidrule(rl){5-6}
				&& Nat. & Cert. & Nat. & Cert. \\
				\midrule
				\multirow{2}*{\mnist}& 0.1 & 99.01 & 98.14 & \textbf{99.15} &  \textbf{98.37}\\
				& 0.3 & 98.46 & 93.40 & \textbf{98.53} &  \textbf{93.51}\\
				\cmidrule(rl){1-6}
				\multirow{2}*{\cifar}& 2/255 & 67.72 & 56.94 & \textbf{79.76} &  \textbf{62.98}\\
				& 8/255 & \textbf{54.84} & \textbf{40.39} & 52.82 &  34.65\\
                \cmidrule(rl){1-6}
                \TIN & 1/255 & 25.69 & 18.18 & \textbf{28.98} &  \textbf{22.16}\\
				\bottomrule
			\end{tabular}
			\label{tab:sort_results}
		\end{threeparttable}
	}
	% \vspace{-1mm}
\end{wraptable}


